Inference Graphs for CNN Interpretation

Convolutional neural networks (CNNs) have achieved superior accuracy in many visual related tasks. However, the inference process through intermediate layers is opaque, making it difficult to interpret such networks or develop trust in their operation. We propose to model the network hidden layers activity using probabilistic models. The activity patterns in layers of interest are modeled as Gaussian mixture models, and transition probabilities between clusters in consecutive modeled layers are estimated. Based on maximum-likelihood considerations, nodes and paths relevant for network prediction are chosen, connected, and visualized as an inference graph. We show that such graphs are useful for understanding the general inference process of a class, as well as explaining decisions the network makes regarding specific images.

==> sections/method/vis_techniques.tex <==
\subsection{Visualization Techniques}\label{subsec:vis_techniques}
We consider several visualization systems, starting from simple visual word to path inference, relating to the different types of networks.

\subsubsection{Simple Cluster}\label{subsubsec:cluster_vis}

We visualize a cluster $C^l_k$ by showing the $m$ examples ($m=6$) with the highest $P(h^l=k | x^l)$.
%Each cluster contains a group of spatial examples according to the GMM. We define that example $x^l$ is \textit{assigned} to cluster $k$ by the following rule
%\begin{equation}
%\label{eq:example_assigned_to_cluster}
  %  h^l = \argmax_{k}P(h^l=k | x^l)
%\end{equation}
%To represent a cluster, we chose the 6 examples with the highest $P(h^l=k | x^l)$.
% \ie the examples in layer $l$ which belong to cluster $k$ the most.
For FC layers, for each representative example, the full image is drawn.
For convolutional layers, visual word examples are typically sub-regions of the input image (if the receptive field does not cover the image entirely). For receptive fields larger than $5\%$ of the image size, the visual word occurrence is visualized by drawing the relevant image with a rectangle around the relevant receptive field (see Fig.~\ref{fig:intro}). When the receptive field is smaller, only the region of the receptive field is drawn instead of the entire image.   

\subsubsection{Cluster as a Decision Junction}\label{subsubsec:DJ_vis}
\begin{figure}[!t]
     \centering
     \includegraphics[width=2.7in]{images/MNIST_DJ.PNG}
    \caption{\footnotesize{\bf Decision Junctions}. Two clusters from a six-layer MLP network trained on the MNIST data. The two images on the left visualize a cluster from Layer 1, and the images on the right a cluster from Layer 2. The top images show sub-cluster representatives chosen by the generative $l_2$ method, and the bottom images by the discriminative $LLR$ method. Each image represents a cluster according to the decision it makes among consecutive cluster alternatives colored in different shades. Transition probabilities to consecutive clusters are stated in the legend. In the left cluster, decision is made between curvy and straight $7$ digits. In the right cluster, decision is made mainly based on the $2$ digits widths and lower part rounds. In both cases, selecting representatives with the $LLR$ criterion provides more extreme examples, enabling easier understanding of the sub-cluster nature.
    % The two images on the left visualize a cluster from layer 2, and the images on the right a cluster from layer 3. The top images show sub-cluster representatives chosen with the generative $l_2$ criterion, and the bottom images use the discriminative $LLR$ criterion. Each image represents a cluster according to the decision it makes among subsequent cluster alternatives colored in different shades. Transition probabilities to subsequent clusters are stated in the legend. In the right cluster decsion is made between curvy end and straight lines of the '$7$' digit. In the left cluster decsion is made based on the closing shape of the upper circle and right tilt direction of the $8$ digit. In both cases, choosing representatives with the $LLR$ criterion provides more extreme examples, enabling easier understanding of the sub-cluster nature.
    }
    \label{fig:DJ_vis}
\end{figure}

%  We suggest present the transition between two consecutive layers as a discrete routing decision using our model. 
In MLP networks, the entire layer activity is assigned to a single cluster. For each cluster $C^l_k$, we consider the clusters in layer $l+1$ to which examples of $C^l_k$ are assigned, where the cluster is considered a decision junction among these subsequent stage choices.
%With this technique, we suggest to represent a cluster of intermediate layer activities, as a local Decision Junction (DJ). This representation can be explained in the following sense: for each example assigned to cluster $k$, as presented in Eq. \ref{eq:example_assigned_to_cluster}, the network "decides" to which cluster it should be assigned in the next layer. We hence propose to represent each cluster as a local DJ, displaying the separation of the activities based on their next-layer cluster label.
% While the transition between two consecutive layers is a complex mapping between two continuous high-dimensional vectors, we can present it as a discrete routing decision using our model. An activity cluster in an intermediate layer, can be seen as a local Decision Junction (DJ) in the following sense: for each example assigned to it (as presented in Equation \ref{eq:example_assigned_to_cluster}), the network decides to which cluster it should be assigned in the next layer. This is a discrete decision. We hence suggest to represent each cluster as a local DJ, displaying the partition of its input space between next-layer labels.

For the visualization of such a decision, the activity vectors assigned to $C^l_k$ using a validation set are labeled according to their cluster index in the consecutive layer, and thereby forming sub-clusters.
% We refer to such labeled sets as \textit{sub-clusters} of cluster $k$.
We use linear discriminant analysis (LDA) \cite{izenman2013linear,fukunaga1990introduction} to find a two dimensional projection of the activities that maximizes the separation of the examples with respect to their sub-cluster labels. 
%The result is a 2D  scatter plot of the data showing sub-cluster separation.
To understand the semantics of the sub-clusters, we draw three representative examples from each sub-cluster near the sub-cluster center position.
%(after LDA projection) in addition to the scatter plot. 
Two methods were considered for selecting the representative examples: 

\begin{enumerate}[leftmargin=*]
\item \textbf{Most typical examples ($l_2$):} The \textit{m} closest images to the sub-cluster center according to the $l_2$ distance.
\item \textbf{Most discriminative examples ($LLR$):}  Assume $C^l_k$  contains $Z$ sub-clusters corresponding to cluster indices $(a_1,...,a_Z)$ in the consecutive layer. For an example $x$ assigned to sub-cluster $a_j$, the log-likelihood ratio (LLR) w.r.t sub-cluster $a_z, ~z\ne j$ is given by
\begin{equation}
LLR(j,z)= \mathrm{log} P\left(x^{l+1}\mathrel{\left|\vphantom{x^{l+1} h^{l+1}=a_j}\right.\kern-\nulldelimiterspace}h^{l+1}=a_j\right)
-{\mathrm{log} P\left(x^{l+1}\mathrel{\left|\vphantom{x^{l+1} h^{l+1}=a_z}\right.\kern-\nulldelimiterspace}h^{l+1}=a_z\right)}
\end{equation}

Since we want the representative examples of sub-cluster $a_j$ to be discriminative w.r.t every other sub-cluster $a_z$, we choose them according to
\begin{equation}
\max\limits_{\{I: h^l(I)=k, h^{l+1}(I)=a_j\} } \min\limits_{ z \ne j}  LLR(j,z)
\end{equation}
\end{enumerate}
The $l_2$ method chooses examples most characteristic of the sub-cluster, while the LLR method focuses on more discriminative, hence extreme examples. See Fig.~\ref{fig:DJ_vis} for decision junction examples.

\begin{figure*}[t]
% \renewcommand{\arraystretch}{1.3}
\begin{center}
\begin{tabular}{c c c c c}
\footnotesize Car & \footnotesize fc-2 & \footnotesize fc-3 & \footnotesize fc-4 \\
% & \multicolumn{1}{p{1.5cm}}{\centering\footnotesize fc-6\\ \footnotesize{Truck class}} 

\raisebox{-.5\height}{\includegraphics*[width=0.25in,keepaspectratio=true]{./images/car.jpg}} $\rightarrow$ &
% \raisebox{-.5\height}{\includegraphics*[width=0.8in,keepaspectratio=true]{./images/Car_Layer1.jpg}} &
\raisebox{-.5\height}{\includegraphics*[width=0.9in,keepaspectratio=true]{./images/Car_Layer2_v3.jpg}} $\rightarrow$ & 

\raisebox{-.5\height}{\includegraphics*[width=1.3in,keepaspectratio=true]{./images/Car_Layer3_v3.jpg}} $\rightarrow$ &

\raisebox{-.5\height}{\includegraphics*[width=1.1in,keepaspectratio=true]{./images/Car_Layer4_v3.jpg}} 
 &
$\longrightarrow$ Truck
\end{tabular}

\end{center}
\begin{flushleft}
\caption{\footnotesize {\bf MLP Inference path}. A main decision junction of a misclassified CIFAR10 car example (presented on the left) passed through six layer MLP network. Each cluster is visualized using its most typical images. In each decision junction, the chosen sub-cluster chosen is marked in turquoise. The main decision points occurred in layers fc-$2$-fc-$4$, with the critical decision made in layer fc-$3$ where the abnormal appearance of the example misled the network to consider the car as a truck.
} \label{fig:Sequential_path}
\end{flushleft}

 \end{figure*}



\subsubsection{Inference Graphs}\label{subsubsec:inferenceGraph}
%The model defined introduces a set of activity clusters in each modeled layer, with transition probabilities estimated between them. It hence allows the definition of a path as the sequence of clusters traversed by an example or set of examples as it progresses through the network.

%\begin{enumerate}
%    \item \textbf{Sequential Path:}
For MLP networks, the inference path of a specific example $I$ connects a single visual word at each layer. It can be defined by the maximum a-posterior (MAP) cluster sequence, i.e., the sequence $H=(h^1,...,h^L)$ satisfying 
    \begin{equation}
    \max_{h^1,...,h^L} \log{P(h^1,...,h^{L} | X(I) ) } 
    \label{eq:Viterby}
    \end{equation}
   $H$ can be found using the Viterbi algorithm~\cite{forney1973viterbi}. The path nodes are visualized using the decision junction technique of Section~\ref{subsubsec:DJ_vis}.
    % \newline
%    \item \textbf{Inference Graph:} 

For CNNs, multiple spatial words are active at each layer. We use the technique explained in Section~\ref{subsec:MWandI} (Algorithm 1) to generate inference graphs highlighting the main active words. Such graphs can be built for an entire class by choosing to input $\Omega$, the set of images predicted to belong to the class, or for a single example. In the visualization of such graphs, each visual word is displayed using its $m$ most representative spatial examples in the validation set. Connections between words are characterized by their contribution to the maximum likelihood (Eq.~\ref{eq:OmageScore}) and using a heat map showing the spatial distribution of explaining words in the receptive field of the target word. For inference graphs for a specific image $I$, node visualization shows spatial locations in $I$ that belong to the node.   
%we provide a sub-graph analysis tool called \textit{Inference Graph}. This sub-graph is created according to an analysed instant; image or class (set of images). The sub-graph is built according to the maximum likelihood based nodes selection \ref{subsec:node_selelction}, visualizing the graph nodes with simple cluster visualization technique \ref{subsubsec:cluster_vis}. The arrows between nodes are colored in different shades indicating the nodes connection strength. We define \textit{'strong'} connection if the log term in ML explanatory power is greater than $1$. \textit{'Weak'} connection is defined by the same log term greater than $0$ and smaller than $1$. On the arrow, we present heatmap indicating the position of the lower visual word in relation to the higher visual word to which it connects. In other words, the heatmap represent the lower visual word location in the receptive field of the higher. For further work, we wish to build a browsing tool over larger graphs, enabling to analyze a wider range of visual words in each layer.
%\end{enumerate}


